DLME: Deep Local-flatness Manifold Embedding

Manifold learning (ML) aims to seek low-dimensional embedding from high-dimensional data. The problem is challenging on real-world datasets, especially with under-sampling data, and we find that previous methods perform poorly in this case. Generally, ML methods first transform input data into a low-dimensional embedding space to maintain the data's geometric structure and subsequently perform downstream tasks therein. The poor local connectivity of under-sampling data in the former step and inappropriate optimization objectives in the latter step leads to two problems: structural distortion and underconstrained embedding. This paper proposes a novel ML framework named Deep Local-flatness Manifold Embedding (DLME) to solve these problems. The proposed DLME constructs semantic manifolds by data augmentation and overcomes the structural distortion problem using a smoothness constrained based on a local flatness assumption about the manifold. To overcome the underconstrained embedding problem, we design a loss and theoretically demonstrate that it leads to a more suitable embedding based on the local flatness. Experiments on three types of datasets (toy, biological, and image) for various downstream tasks (classification, clustering, and visualization) show that our proposed DLME outperforms state-of-the-art ML and contrastive learning methods.

==> Sec_withcontrastiveLearning.tex <==

\begin{figure*}[t]
  \centering
  \includegraphics[width=5.5in]{figs/FIg-Intro.pdf}
  \caption{
Structural of deep manifold learning, self-supervised contrastive learning and our proposed DSML.
(a) {\bf Deep manifold learning} calculates the similarity $S^x$ and $S^z$ in the input space and latent space, and then trains the neural network $f_\theta(\cdot)$ using the matching degree of similarity as the loss function.
(b) {\bf Self-supervised contrastive learning} assuming that data augmentation does not change the semantics of the data, generates augmentation data pairs $(v_i,v_j)$ from the original data $x$, and then trains the neural network $f_\theta(\cdot)$ by maximizing the similarity between positive pairs (from same original data) and minimizing the similarity between negative pairs (from different original data).
(c) {\bf DSML} uses two networks $g_{\bar \theta}, f_{\theta}$ components to map the augmentation data $(v_i,v_j)$ to points semantic space $(z_i, z_j)$ and the embedding space $(e_i, e_j)$. Then the semantic similarity of positive sample pairs is improved by semantic scaling and traveling semantic distance, and finally both networks are trained simultaneously by matching the similarity loss.
  }
  \label{fig:FIg-Intro}
\end{figure*}

\textbf{Deep manifold learning}, as shown in Figure \ref{fig:FIg-Intro} (a), trains a mapping $f_\theta(\cdot): x \in \mathbb R^{ \mathcal{M} } \rightarrow  z \in \mathbb{R}^{m}, m < \mathcal{M}$ that $\theta$ is the parameter of the network, thus, we have $z = f_{\theta}\left(x\right)$. 
Almost all of the manifold learning methods are under the \emph{local connectivity assumption}, meaning that the resulting topological structure derived from the manifold is locally connected\cite{mcinnes_umap_2018,lee_shift-invariant_2011}. In practice, this can be realized by measuring distance in the extended pseudo-metric space local to $x_i$ as geodesic distance beyond the nearest neighbor of $x_i$.
For easy comparison, we rewrite the loss function $\mathcal{L}_{\text{dml}}$ of \cite{maaten_learning_2009,maaten_visualizing_2008} as:
\begin{equation}\label{eqn:tsne}
  \begin{aligned}
    &\mathbb{E}_{
      \substack{x_i, x_j, \{{x_k^b}\}_{k=1}^N }
      }
    \left [ 
        \mathcal{\widetilde{S}}(x_i,x_j) \log \frac{\mathcal{\widetilde{S}}(x_i,x_j)}{\mathcal{\widetilde{S}}(f_\theta(x_i), f_\theta(x_j))}
        \right 
    ]\!, \\
    &\mathcal{
      \widetilde{S}
      }
    (x_i,x_j)=\frac{\mathcal{{S}}(x_i,x_j)}{\mathcal{{S}}(x_i,x_j)+\sum_k \mathcal{{S}}(x_i,x_k^b)},
      \end{aligned}
 \end{equation}
where $x_i, x_j$ and $\{{x_k^b}\}_{k=1}^N$ are sampled from dataset $\mathcal X$, and 
$\{{x_k^b}\}_{k=1}^N$ are the other samples in a mini-batch excluding $x_i,x_j$, used to normalize the probability $\{{x_k^b}\}_{k=1}^N$, which is named as background samples.
The pair-wise similarity 

\begin{equation}
  \mathcal{S}(x_i,x_j)=\kappa( d(x_i, x_j), \sigma)=e^{d(x_i,x_j)^2/-\sigma^2}, 
\end{equation}

where $d(x_i, x_j)$ is a distance metric for $x_i$ and $x_j$, using Euclidean distance by default. $\kappa(\cdot)$ is a kernel function to convert the distance into the similarity of the nodes, the closer the distance, the greater the similarity. More complex kernel functions may be used in practical applications.
To show its essence, we rewrite Eq.(\ref{eqn:tsne}), keeping only the parts that are meant for optimizing the network parameters $\theta$.

\begin{equation} \label{eqn:dml_tsne_2}
  \begin{aligned}
  &\mathbb{E}_{
    \substack{x_i, x_j, \{{x_k^b}\}_{k=1}^N}
    }\!\bigg[ -
    % \underbrace{
      % \frac {\mathcal{S}(x_i,x_j)}{\mathcal{S}(x_i,x_j)\!+\!\sum_k \mathcal{S}(x_i,x^b_k)}
      P_{ij}
      % }_{\text{(A): Similarity Target (soft label)}} \log 
    % \underbrace{
      \log{Q_{ij}}  
    % \frac
    %   {
    %     \mathcal{S}(f_\theta(x_i), f_\theta(x_j))
    %     }
    %   {
    %     \mathcal{S}(f_\theta(x_i), f_\theta(x_j))\!+\!
    %     \sum_k \mathcal{S}(f_\theta(x_i), f_\theta(x^b_k))
    %   }
      % }_{ \text{(B): Similarity Output}}
      \!\bigg].\\
      &P_{ij} =\frac {\mathcal{S}(x_i,x_j)}{\mathcal{S}(x_i,x_j)\!+\!\sum_k \mathcal{S}(x_i,x^b_k)} \\
      &Q_{ij} =  \frac
        {
          \mathcal{S}(f_\theta(x_i), f_\theta(x_j))
          }
        {
          \mathcal{S}(f_\theta(x_i), f_\theta(x_j))\!+\!
          \sum_k \mathcal{S}(f_\theta(x_i), f_\theta(x^b_k))
        }
  \end{aligned}
\end{equation}

Eq.\ref{eqn:dml_tsne_2} is a special form of Bregman divergence\cite{zang_unsupervised_2021}, where the goal of optimization is to make A (Similarity Target) and B (Similarity Output) as close as possible.


\textbf{Self-supervised contrastive learning} introduces a new assumption that \emph{data augmentation do not change the data's semantic}\cite{chen2020simple}. The key idea is to contrast semantically similar (positive) and dissimilar (negative) pairs of data points, encouraging the representations of similar pairs $(x, x^+)$ to be close, and those of dissimilar pairs $(x,x^-)$ to be more orthogonal \citep{oord2018representation, chen2020simple}, The loss function can be written as:
\begin{equation}
  \begin{aligned} \label{eqn:nce}
    \mathcal{L}_{\text{scl}} & = 
    \mathbb{E}_{\substack{x, x^+, \{x^-_i\}_{i=1}^N}}
    \bigg[
      - 
      % \underbrace{1}_{\text{(A): Similarity Target (soft label)}}
      \log 
      % \underbrace{
      Q_{ij}  
        % }_{\text{(B): Similarity Output}} 
    \bigg]. 
    \\
    Q_{ij} &= \frac{e^{g_{\bar \theta}(x)^T g_{\bar \theta}(x^+)}}{e^{g_{\bar \theta}(x)^T g_{\bar \theta}(x^+) } + \sum_{i=1}^N e^{g_{\bar \theta}(x)^T g_{\bar \theta}(x_i^-)} }
  \end{aligned}
\end{equation}

where $g_{\bar \theta}(x^+)$ is a network mapping function. In practice, the expectation is replaced by the empirical estimate. For each training data point $x$, it is common to use one positive example, e.g., derived from perturbations, and $N$ negative examples $x^-_i$. The loss function concentrates on the positive samples and the negative samples play a similar role to the background samples in Eq. (\ref{eqn:dml_tsne_2}).

{\bf Similarities and differences between the two methods.} 
We are surprised to find that the Eq. (\ref{eqn:dml_tsne_2}) and Eq. (\ref{eqn:nce}) are very similar, with similarities including:
\begin{itemize}
  \item Both loss functions handle the similarity between samples by negative logarithms.
  \item The denominator is a normalization of the numerator to prevent the collapse of the mapping.
  \item Both numerators describe the similarity of sample pairs in the latent space.
\end{itemize}
The substantial difference between the two losses is the coefficients in front of the exponential term. The coefficients of deep manifold learning are $\frac {\mathcal{S}(x_i,x_j)}{\mathcal{S}(x_i,x_j)\! +\! \sum_k \mathcal{S}(x,x^b_k)}$, which takes the similarity of the input space as the goal to fit. And the coefficient of self-supervised contrastive learning is $1$, which means maximizing the similarity between positive sample pairs.

{\bf The challenge of the deep manifold learning method} is when the input manifold is too complex or too sparsely sampled, which destroys the critical assumption of deep manifolds (local connectivity assumption), resulting Eq. (\ref{eqn:dml_tsne_2})'s (A) failing to obtain a reasonable learning objective, thus invalidating the whole method.
{\bf The challenge of the self-supervised contrastive learning method} is the false negative samples. Since true labels or true semantic similarity are typically not available, negative counterparts $x^-_i$ are commonly drawn uniformly from the training data. But, this means it is possible that $x^-$ is similar to $x$. This phenomenon, which we refer to as \textit{false negative problem}, can empirically lead to a significant performance drop. 
However, the ideal unbiased objective is unachievable in practice since it requires knowing the labels, i.e., \emph{supervised} learning. This dilemma poses whether it is possible to reduce the gap between ideal and standard contrastive learning without supervision. 


==> p_fig_abla_batchsize.tex <==
\begin{figure}[]
    \centering
    \includegraphics[width=3.2in]{figs/ab1.pdf}
    \caption{
        The relationship between the number of samples in the batch and the training accuracy (CIFAR100 linear test for 1000 Epochs
    }
    \label{fig:i}
% \vspace{-4pt}
\end{figure}

==> p_tab_nlpacc.tex <==
\begin{table}
    \caption{Classification accuracy on 3 downstream tasks.}
    \small
    \centering
    \begin{tabular}{@{}ccccccccc@{}}
        \toprule
        Method              & MR            & CR            & SUBJ          \\ \midrule
        QT                  & 76.8          & 81.3          & 86.6          \\
        Debiased            & 76.2          & 82.9          & 86.9          \\
        HARD                & 77.1          & \textbf{83.6} & 86.8          \\ \midrule
        \textbf{DSML}       & \textbf{77.3} & \textbf{83.6} & \textbf{87.1} \\ \bottomrule
    \end{tabular}
\end{table}
